zksk: A Library for Composable Zero-Knowledge Proofs

Zero-knowledge proofs are an essential building block in many privacy-preserving systems. However, implementing these proofs is tedious and error-prone. In this paper, we present zksk, a well-documented Python library for defining and computing sigma protocols: the most popular class of zero-knowledge proofs. In zksk, proofs compose: programmers can convert smaller proofs into building blocks that then can be combined into bigger proofs. zksk features a modern Python-based domain-specific language. This makes possible to define proofs without learning a new custom language, and to benefit from the rich Python syntax and ecosystem. The library is available at https://github.com/spring-epfl/zksk

==> figures/rw-table.tex <==
\begin{table*}[htb]
  \newcommand{\yes}{\checkmark}
  \newcommand{\no}{$\times$}
  \caption{\label{tab:comparison}Comparison between different zero-knowledge
    proof libraries. Columns:
    \emph{AND, OR} -- support for conjunct and disjunct statements,
    \emph{Composing} -- defined statements compose into bigger statements,
    \emph{Interactive} -- interactive prove/verification mode,
    \emph{FS} -- non-interactive proofs through Fiat-Shamir heuristic,
    \emph{Language} -- language in which the tool is implemented,
    \emph{DSL} -- language in which proofs can be defined,
    \emph{Documentation} -- available
    documentation.}
  \begin{tabular}{lcccccccc}
    \toprule
    & AND & OR & Composing & Interactive & FS & Language & DSL &  Documentation \\
    \midrule
    Emmy~\cite{emmy} & \no & \no & \no & \yes & \no & Go & - & \no \\
    zkp~\cite{dalek} & \yes & \no & \no & \no & \yes & Rust & Rust & minimal \\
    Cashlib~\cite{MeiklejohnEKHL10} & \yes & \no & \no & \no & \yes & C++ & Custom & \textasciitilde \\
    YAZKC~\cite{AlmeidaBBKSS10} & \yes & \yes & \no & \yes & \yes & C & Custom & \textasciitilde \\
    SCAPI~\cite{EjgenbergFLL12,SCAPI} & \yes & \yes & \textasciitilde & \yes & \yes & C++ & C++ & \yes \\
    \name (this work) &  \yes & \yes & \yes & \yes & \yes & Python & Python & \yes \\
    \bottomrule
  \end{tabular}
\end{table*}

